Extremum-Seeking Adaptive-Droop for Model-free and Localized Volt-VAR Optimization

In an active power distribution system, Volt-VAR optimization (VVO) methods are employed to achieve network-level objectives such as minimization of network power losses. The commonly used model-based centralized and distributed VVO algorithms perform poorly in the absence of a communication system and with model and measurement uncertainties. In this paper, we proposed a model-free local Volt-VAR control approach for network-level optimization that does not require communication with other decision-making agents. The proposed algorithm is based on extremum-seeking approach that uses only local measurements to minimize the network power losses. To prove that the proposed extremum-seeking controller converges to the optimum solution, we also derive mathematical conditions for which the loss minimization problem is convex with respect to the control variables. Local controllers pose stability concerns during highly variable scenarios. Thus, the proposed extremum-seeking controller is integrated with an adaptive-droop control module to provide a stable local control response. The proposed approach is validated using IEEE 4-bus and IEEE 123-bus systems and achieves the loss minimization objective while maintaining the voltage within the pre-specific limits even during highly variable DER generation scenarios.

==> name/oldsection2-3.tex <==


\section{Proposed Extreme Seeking based Volt-VAR Optimization (VVO)  (Preliminaries)}
%We define the general problem of Volt-VAR optimization (VVO) in power distribution system and introduce the proposed local control architecture for VVO with the objective of loss minimization. %The comprehensive proposed algorithm flow is shown in Fig. \ref{fig:proposedvvo}.

%\subsection{Problem Description}
The problem objective is to minimize the total power loss for an unbalanced power distribution system while maintaining the nodal voltages within ANSI \cite{ANSI} limits using only local control of the reactive power dispatch from the smart inverters. %That is, we aim at designing the algorithms for decision-making on reactive power generation $Q_{PV}(t)$, noted as $q$ for simplicity, by  using only local measurements to achieve a combine objective of
The notional problem formulation is stated in (\ref{Objective}). % and (\ref{fVpen}). 


\begin{equation}
\small
\label{Objective}
\underset{V_{ref}}{\text{minimize:}} \hspace{0.2 cm} \sum_{{ij} \in \mathcal{E}}I_{ij}^2(t) r_{ij}  + \sum_{i \in \mathcal{N}} f_{Vpen}(V_i(t))   
\end{equation}
where:
\begin{flalign}\label{fVpen}
\small
\nonumber   f_{Vpen}(V_i(t))=
  \begin{cases}
    (0.95-V_i(t)) \times K_{p} &\text{ $ V_i(t) \leq 0.95 $ } \\
    \ \ \ 0                  &\text{ $0.95 < V_i(t) < 1.05$ } \\
    (V_i(t)-1.05)\times K_{p} &\text{ $V_i(t) \geq 1.05$} \\
 \end{cases}
\end{flalign}
$\mathcal{N}$ and $\mathcal{E}$ represent the set of nodes and lines/edges in the distribution system, respectively; $V_i(t)$ is the voltage at node $i$ at time $t$; $I_{ij}(t)$ is the current flow in line $(ij)$; $r_{ij}$ is the resistance of the branch $(ij)$; $K_p$ is the weighing factor for the voltage violation penalty function, $f_{Vpen}(V_i(t))$. $K_p$ should be of the same as $I^2$ to weight voltage penalty. %Here, $K_p = 10^{log(I^2)+k}$, where, $k$ is set between 3 and 5.

%If selected $K_p$ is much smaller than $I^2$, the objective function would be unable to drive the voltage profile back to acceptable range. We can use the magnitude of $I^2$ term and the pu value of the voltage to determine voltage penalty weight $K_p$, and $K_p$ is close to $10^{log(I^2)+k}$. In this paper, $k$ is set between 3 and 5.


%\end{minipage}
%\vspace{0.2cm}

%Here, to avoid voltage violation beyond control range of original droop based VVC, the inequality constraints are transferred to voltage penalty function and included in combined objective function. 

% \textcolor{red}{can we cite it?} \textcolor{blue}{removed "Generally"}

% Due to the linear droop VVC mapping between $V_t$ at a node  and reactive power generation $q$, the voltage penalty function is convex wrt $q$ and it does not change the convexity of the combined objective function. 

\begin{comment}
\begin{figure}[t]
\includegraphics[width=.9\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{Images/VVCdroopQ0.eps}
\vspace{-0.2cm}
	\caption{$Q_0$ adjustment in Volt-VAR control \cite{singhal2018real}}
\vspace{-0.2cm}
	\label{fig:Q0Adjust}
\end{figure}
\end{comment}

%As recommended by IEEE 1547 standard \cite{8332112}, PVs with smart inverters have the capability to control their active and reactive power dispatch. This has motivated 

One popular approach in related literature is to employ droop-based local Volt-VAR control (VVC) methods where the reactive power output from the smart inverters change as a function of local nodal voltages to manage the feeder voltages within the specified ANSI limits. The traditional droop-based methods, however, do not achieve network-level objectives such as loss-minimization. For network-level optimization, existing literature presents centralized, distributed, and decentralized methods. However, these require network model and communication with other to achieve the problem objective. The objective of this paper is to employ local measurement-based control for network-level optimization. To this regard, we review extremum seeking algorithm that is a measurement-based local control approach to obtain for optimizing a problem objective. For fast changing phenomenon, a large number of extremum-seeking controllers may lead to hunting effects and instability. This calls for other control loops to mitigate the challenges with fast-changing phenomenon. Adaptive droop-control is effective in such cases. In what follows, we introduce Droop-based VVC and extremum seeking optimization methods.

%an adaptive droop VVC and build local optimization upon that to generate desired reactive power. First we check the parameters, $V_{min}, V_{max}, V_{ref}, Q_{min}, Q_{max}, Q_0$, which are required to determine a droop curve as shown in Fig. \ref{fig:Q0Adjust}. The $Q_{min}, Q_{max}$ are determined by the kVA rating of the smart inverter  and active power output of a PV at a given time from eq (\ref{eqQmax}). The value for $V_{min}, V_{max}$ are the adjustable parameters which are specified in IEEE 1547 standard \cite{8332112}. $V_{ref}$ is the voltage reference and $Q_0$ is the reactive power reference obtained from the optimization problem. 

% operation where the objective is to maintain nodal voltage while load demand, feeder head voltage or any other states changes in the system.

%The reactive power injection from PVs will have impact on power flow distribution, and further derive voltage and power loss changes. For purely local design, the reactive power generation is determined by local droop based VVC, whose purpose is to maintain nodal voltage while load demand, feeder head voltage or any other states changes in the system.

\vspace{-0.3cm}

%\subsection{Background}



\subsubsection{Extremum seeking optimization}
Extremum seeking is a measurement-based real-time local control method that seeks optimum of a function without requiring the model parameters or communication with other nodes. A sinusoidal signal, $sin({\omega}t)$, is used as a time continuous perturbation to the physical system to estimate gradient of the objective function.  The overall approach is detailed in Fig 2. The system measurements are used to estimate current value of the objective function, $y$, that needs to be optimized. The estimate of the objective function, $y$, is passed through a washout filter to remove noise having frequency component lower than $\omega_h$. The resulting signal is multiplied with the sinusoidal perturbation and passed through an integrator with gain $K$. The resulting signal, $\hat{u}$ is then lead to a smaller gradient direction. The scheme will converge to local minimum when $K > 0$. Otherwise, the scheme will converge to local maximum. 

\begin{comment}
The mathematical representation of the extremum seeking scheme is  given in  (5) -(7). 
\begin{eqnarray}\label{eqES1}
\small
   \dot{y}  = \dot{\eta}-h\eta\\
   \label{eqES2}
    \dot{\hat{\mu}}=-K*Asin (\omega t)*\eta\\
    \label{eqES3}
    \mu=\hat{\mu}+Asin\omega t
\end{eqnarray}
\end{comment}

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{Images/SeekingConceptsimpleflow.eps}
\vspace{-0.2cm}
	\caption{Extreme Seeking Scheme \cite{liu2012stochastic}}
\vspace{-.1cm}
	\label{fig:ESflow}
\end{figure}


\begin{figure}[t]
\includegraphics[width=0.45\textwidth]{Images/ExtremeSeekingConcept}
\vspace{-0.2cm}
	\caption{Extreme Seeking Scheme Concept \cite{KRSTIC2000595}}
\vspace{-0.2cm}
	\label{fig:ESschemeConcept}
	\vspace{-0.5cm}
\end{figure}



{\color{red} This paragraph is not clear. Also, Fig. 3 is not clear. YOu need to represent the perturbation and response in terms of same variables you use in Fig. 2 for clarity. 

Fig. \ref{fig:ESschemeConcept} illustrates the principle of the extremum seeking algorithm to estimate gradient and reach local maximum point of unknown function. Here,  $\mu^*$ is the maximum of the function, which is the target of the extremum scheme.
When the initial guess $\mu_1$ is in the left side of the  $\mu^*$, the response is in opposite phase with perturbation signal. The integration of the product of perturbation $Asin({\omega}t)$ and response is negative which eliminates the DC component of the product through washout filter. The integration, of a negative number and multiplied with negative constant K to obtain positive values to drive the next estimation of $\mu_1$ closer to the optimal value $\mu^*$. Finally, the integration will be close to zero when $\mu_1$ is close enough to the  $\mu^*$. If the initial guess is on the other side like $\mu_2$, the similar estimation process will drive the next guess closer to the optimal value $\mu^*$.}

\subsubsection{Adaptive Droop-based VVC scheme} The droop-based VVC uses a linear mapping from nodal voltages, $V_i$ and respective nodes reactive power generation, $Q_{i,dp}$, see (\ref{eqQdp}). Compared to the conventional VVC, an adaptive VVC allows for the parameters, $Q_0$ and $V_{ref}$ in (\ref{eqQdp}) to be adjustable (see Fig. \ref{fig:VrefAdjust}). In the proposed approach, $V_{ref}$ is determined and periodically updated by a local extremum seeking optimization method to achieve network-level optimization. 


%for slope between $V_{min}$ and $V_{ref}$, and the slope on the other side can be adjusted by $Q_0$ (see Fig. \ref{fig:Q0Adjust}). It means adjusting $Q_0$ can mitigate potential instability by changing droop slopes as well as reduce steady state error. 
%Similarly, $V_{ref}$ is also time varying (see Fig. \ref{fig:VrefAdjust}). 
% \textcolor{red}{what is meant by upper level? Please specify it. Also, you need to describe eq(3) and (4)  here. What are there function, how it is connected with fig.3 and 4.  In fig.3 and 4 , Vl and Vh is shown, you need to define what  it mean, range of it?} \textcolor{blue}{updated two figures with Vl and Vr}
\vspace{-0.2cm}
\begin{equation} \label{eqQmax}
\small
 Q_{max}(t) =  -Q_{min}(t) = \sqrt{(S_{PV^{rated}})^2 - (P_{PV}(t))^2} 
\end{equation}
\vspace{-0.5cm}
\begin{align*}
\small
      Q_{dp}(t+1) = f(& V_t, V_{min}, V_{max}, V_{ref}(t), DB, ... \\
             &... Q_{min}(t),  Q_{max}(t), Q_0(k_n)) 
\end{align*} 
\vspace{-0.5cm}
\begin{equation}\label{eqQdp}
\small
f(\bullet) = 
\begin{cases}

   \: \: Q_{max}   &\text{if $ V_t \leq V_{min} $ } \\
   -\dfrac{Q_{max}-Q_0}{V_{l}-V_{min}}(V_t-V_{l})+Q_0   &\text{if $V_{min} \leq V_t \leq V_{l}$ } \\
    \: \: Q_0  &\text{if $V_{l} \leq  V_t  \leq V_{r}$} \\
    -\dfrac{Q_{min}-Q_0}{V_{r}-V_{max}}(V_t - V_{r})+Q_0 & \text{if $ V_{r} \leq V_t \leq V_{max}$} \\
    \: \: Q_{min}  &\text{if $ V_t \geq V_{max} $ } \\
\end{cases}
\end{equation}
where, $DB$ stands for dead band. The left side of bead band is $V_{l}= V_{ref}-DB/2$ and the right side $V_{r}= V_{ref}+DB/2$.%, which are shown in Fig.\ref{fig:Q0Adjust}. 



\begin{figure}[t]
\includegraphics[width=.75\columnwidth, trim={0cm 0cm 0cm 0cm},clip]{Images/VVCdroopVref.eps}
\vspace{-0.2cm}
	\caption{$V_{ref}$ adjustment in Volt-VAR control}
\vspace{-.5cm}
	\label{fig:VrefAdjust} 
	\vspace{0.5cm}
\end{figure}


\begin{figure*}[t]
 \centering
\includegraphics[width=0.8\textwidth,height=2.4in]{Images/VVO3.eps}
\vspace{-0.1cm}
	\caption{Proposed Volt-VAR control with optimization}
\vspace{-0.5cm}
	\label{fig:proposedvvo}
\end{figure*}

\begin{figure}[t]
\includegraphics[width=0.5\textwidth, trim={0cm 0cm 0cm 0cm},clip]{Images/Outerloopconcept2.eps}
\vspace{-0.5cm}
	\caption{Inner and outer loop update scheme}

	\label{fig:OuterLoop} 
	\vspace{-0.3cm}
\end{figure}

\section{Proposed Extreme Seeking based Volt-VAR Optimization (VVO)}
Our objective is to design a network-level optimizer using only local control of smart inverters that is also stable and capable of managing fast-changing events. The proposed approach is a combination of (1) a droop control approach employed to ensure a stable operation and to regulate fast-changing generation patterns due to PVs, (2) an extremum seeking approach to achieve the global (network-level) objective of minimizing the feeder loses using local perturbation-based controller, and (3) a static-error correction module to include the effects time-varying load profiles. 

%\subsection{Proposed Extremum Seeking based VVO}
The overall framework is detailed in Fig. 4.  The proposed controller includes three modules: (1) Adaptive Volt-VAR droop control with reactive power inertia; (2) Extremum seeking control for network-level optimization; and (3) static state error adaption (see Fig. \ref{fig:proposedvvo}). First two modules lie in the inner loop and are updated every time-step; each time-step is of 30 sec duration. The static state error adaption is in the outer loop and is updated every $T=10$ time steps, i.e. every 5 min to account for large changes in the system loading. The time-evolution of the controller is shown in Fig.\ref{fig:OuterLoop}. Note that the proposed controller is locally situated at the controllable node, i.e. the node with the smart-inverter.

%In this paper, we assume that time-steps are discretized in 30 secs window; inner loop operates every 30 secs. The nodal measurements $V(t)$, $I(t)$ and $q(t)$ are inputs to the inner loop. The outer loop includes a steady state error adaption function to mitigate impact of the reactive power oscillations caused by setting of $Q_0$. The outer loop runs every $T$ time steps, where $T$ is ten 30-sec time steps (i.e. 5 minutes). The extremum seeking function code in this paper is inspired from  \cite{brunton2019data}. 

%Based on time response of control schemes, we classify fast, medium and slow controls to deal with different time scale changes in system. The detailed explanation of each components is discussed below. 

\subsection{Slow Changes Tracking - Extremum Seeking}
The extremum seeking method is implemented to track optimal solution with continuous small magnitude perturbation in voltage setting $V_{ref}$ in the droop when generations and loads in the system are changing slowly. Here, the frequency excitation signal and parameters of washer filters are identical for all PV inverters in the system. The proposed method is using local objective function, thus, there is no significant cross impact from same frequency perturbations of other PVs as those of different frequency settings in paper \cite{7350258}. 


\subsubsection{Medium Speed Adjustment - Static State Error }
The steady state error (SSE) is defined as the difference between $V_{ref}$ and steady state voltage in (\ref{eqSSE}) which was defined in  \cite{singhal2018real}. By measuring the real time SSE, we can obtain an  adaptive $Q_0$ which helps in mitigating  the reactive power oscillation. The oscillation is caused by significant difference between $Q_0$ setting of droop control and required reactive power $Q_{req}$ to maintain the nodal voltage close to $V_{ref}$ (by default $Q_0$ is zero as per IEEE-1547 standard). However, for load node, it require $Q_{req}$ to raise the voltage to $V_{ref}$. The SSE is used to estimate $Q_{req}$ and set $Q_0$ close to it as well as adjust droop slope accordingly.

The Fig.\ref{fig:VVCunstable}, provides a pictorial representation for the unstability of the droop curve. According to droop curve, the PV will generate reactive power $Q_{V0}$ to raise the node voltage from $V_0$ to $V_1$, which maybe exceed $V_{ref}$ at first time step. In next time step, PV may absorb reactive power $Q_{V1}$ due to the slope of the droop control, which result in voltage drop from $V_1$ to $V_2$, in the third time step. Afterwards, the droop curve will control PV to generate more $Q_{V2}$ to drive system node voltage to $V_{3}$. Thus, the droop control generates or absorbs large reactive power than demand for each time step and cause oscillation. The SSE reduces the gap between $Q_{dp}$ and $Q_{demand}$ by setting $Q_0$ and adjusting the slope in Fig.\ref{fig:Q0Adjust}. When $Q_0$ require large change exceeding $Q_{0Large}$ from previous $T$ interval, we will shorten $T$ to $T_small$ = 8 to track fast load changes as shown in Fig. \ref{fig:OuterLoop} and algorithm \ref{alg:ESVVO1}.

\begin{eqnarray}\label{eqSSE}
\small
&SSE(k_n )= \sum_{t=k_nT+1}^{(k_n+1)T} (V_{t}-V_{ref,t})   \\
&Q_0(k_n) = Q_0(k_n-1) -K_Q *SSE(k_n),   k_n=1,2,3 ... 
\end{eqnarray}
% \vspace{0.2cm}
Here, $T$ is 10-20 time steps those are inner loop time length. $K_Q$ is positive number in the same order as the inverter capacity when pu values of voltages are used. 

\begin{figure}[t]
\centering
\vspace{-0.2cm}
\includegraphics[width=0.8\columnwidth, trim={0.3cm 0 0 0},clip]{Images/VVCunstable.eps}
\vspace{-0.2cm}
	\caption{Unstable droop based Volt-VAR control.}
\vspace{-0.2cm}
	\label{fig:VVCunstable}
	\vspace{-0.8cm}
\end{figure}
% \vspace{0.5cm}
%\vspace{-0.5cm}

\subsubsection{Fast Droop Control - VVC modification}
The volt-VAR droop control is required to maintain the voltage within a permissible voltage range. Conventionally, the change in voltage is sensed by the local control, if the node voltage is beyond a permissible value, local control calculate the required reactive power $Q_{dp}$ from smart inverter using the fixed slope. The reactive power support will maintain the voltage withing the limits.  However, the droop control in conventional version may introduce reactive power oscillations due to sharp slope and steady state error \cite{singhal2018real}. Thus, here we introduce reactive power inertia through low pass filter to mitigate sudden large $Q_{dp}$ variance in Fig.\ref{fig:proposedvvo}, and SSE adaption to reduce the setting errors in Fig.\ref{fig:Q0Adjust}.   
The low-pass filter mitigates sudden reactive power changes and oscillation caused by droop control, thus this filter is added after the Volt-VAR droop control scheme \cite{jahangiri2013distributed}. The final reactive power generation is determined by both previous time step reactive power from PV and current Volt-VAR droop control function $Q_{dp}$ result.  
The settings of $V_{ref}, Q_0, Q_{min}, Q_{max} $ are time varying variables, which is different from traditional Volt-VAR control. 
\begin{equation}\label{eqQt}
\small
    Q_{PV}(t+1) = (1-\mu) Q_{PV}(t) + \mu Q_{dp}(t+1)  
\end{equation}
\vspace{-0.4cm}

\begin{comment}


\begin{algorithm}[h]
\small
\caption{\small Localized VVO algorithm}\label{alg:ESVVO}
	%\noindent\rule{8.4cm}{1pt}\\ 
\SetAlgoLined
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
% \SetKwInOut{defi}{define}
\SetKwInOut{init}{initialize}
% \defi{$x = x$}
\Input{V_t,I}
\Output{V_{ref}(t)}
\init{Q_0(0), V_{ref}(t_0),V_{min}, V_{max}} 
\hline
%\noindent\rule{8.4cm}{1pt}
\While {$t$ in range ($t_0, t_{end}$)}{
update $V_{ref}(t)$ from Extremum Seeking function\\
	\If {$t = kT, k = 1,2,3, ...end$}{
        calculate SSE (k)  from eq (6)          \\
        calculate Q_0(k) and limit it in $[Q_{min}, Q_{max}]$      \\
        calculate $Q_{droop}(t) = f(V_t, V_{ref}(t)$  from eq(9)    \\
        calculate Q(t) from eq(7)   \\
        {Increment iteration count, $ k = k+1$} \\
        \If { $|Q_0(k) - Q_0(k-1)| \geq Q_{0,large}$ } {
         reduce outer loop $T$ to $T_{small} $ \\
         \else keep same $T$
        }
        
    \else calculate $Q_{droop} (t) f(V_t, V_{ref}(t), ...$ from eq (9) \\
    calculate Q_{PV}(t) form eq(7) 
        
	}	

}
%	\noindent\rule{8.4cm}{1pt}\\
	\label{algo}
	\vspace{-0.1cm}
\end{algorithm}
\end{comment}

% \vspace{0.35cm}
\begin{algorithm}[h]
\small
\caption{\small Localized VVO algorithm}\label{alg:ESVVO1}
	%\noindent\rule{8.4cm}{1pt}\\ 
\SetAlgoLined
    \SetKwInOut{Input}{input}
    \SetKwInOut{Output}{output}
% \SetKwInOut{defi}{define}
\SetKwInOut{init}{initialize}
% \defi{$x = x$}
\Input{$V_t$, $|I|^2$ or $S_{loss}$}
\Output{$V_{ref}(t)$}
\init{$Q_0(0)$, $V_{ref}(t_0)$, $V_{min}$, $V_{max}$} 
\hline
 \While{t in range ($t_0$, $t_{end}$)}{   
  Update $V_{ref}(t)$ from $ES$ function\;
  \eIf{t = hT, h=1,2,3 ...}{
   Calculate $SSE(k_n)$ from eq(\ref{eqSSE}); \\
   Calculate $Q_0(k_n)$, with limit in [$Q_{min}, Q_{max}$];\\
   Calculate $Q_{dp}(t) = f(V_t, V_{ref}(t), ...)$ from eq(\ref{eqQdp});\\
   Calculate $Q_{PV}(t)$ from eq(\ref{eqQt});\\
   $k_n=k_n+1$;\\
   \eIf{$|Q_0(k_n) - Q_0(k_n-1)| \geq Q_{0Large}$}{
   Reduce outer loop $T$ to $T_{small}$\;
  % instructions2\;
   }{
   Keep same $T$\;
  }
  }
  {
    Calculate $Q_{dp}(t) = f(V_t, V_{ref}(t), ..)$  from eq(\ref{eqQdp});\\
    Calculate PV output $Q_{PV}(t)$ from eq(\ref{eqQt});
  }
  $V_{ref}(t)$ =  ExtremumSeeking($|I|^2 \ or \ S_{loss} + f_{Vpen}$) \\
  ES function refers to eq(\ref{eqES1}, \ref{eqES2}, \ref{eqES3}) and discrete time sample in \cite{brunton2019data} and search range of $V_{ref}(t)$ is [0.95, 1.05]
 }
\end{algorithm}
\vspace{-0.1cm}
